The computation of approximate feedback Stackelberg equilibria in multi-player nonlinear constrained dynamic games

Solving feedback Stackelberg games with nonlinear dynamics and coupled constraints, a common scenario in practice, presents significant challenges. This work introduces an efficient method for computing approximate local feedback Stackelberg equilibria in multi-player general-sum dynamic games, with continuous state and action spaces. Different from existing (approximate) dynamic programming solutions that are primarily designed for unconstrained problems, our approach involves reformulating a feedback Stackelberg dynamic game into a sequence of nested optimization problems, enabling the derivation of Karush-Kuhn-Tucker (KKT) conditions and the establishment of a second-order sufficient condition for local feedback Stackelberg equilibria. We propose a Newton-style primal-dual interior point method for solving constrained linear quadratic (LQ) feedback Stackelberg games, offering provable convergence guarantees. Our method is further extended to compute local feedback Stackelberg equilibria for more general nonlinear games by iteratively approximating them using LQ games, ensuring that their KKT conditions are locally aligned with those of the original nonlinear games. We prove the exponential convergence of our algorithm in constrained nonlinear games. In a feedback Stackelberg game with nonlinear dynamics and (nonconvex) coupled costs and constraints, our experimental results reveal the algorithm's ability to handle infeasible initial conditions and achieve exponential convergence towards an approximate local feedback Stackelberg equilibrium.

==> siam_tex/kkt_condition_old.tex <==
\section{Necessary and Sufficient Conditions for Local Feedback Stackelberg Equilibria}

% \begin{definition}[Linear Independence Constraint Qualification (LICQ)]
%     Let $x\in\mathbb{R}^{(T-1)Nn}$ and $u\in\mathbb{R}^{TNm}$ be the state and control trajectory under a feedback Stackelberg strategy to a Stackelberg game defined by \eqref{eq:dynamics}, \eqref{eq:costs}, \eqref{eq:constraints at t} and \eqref{eq:terminal constraints}. Let the set of active inequality constraints at $(x,u)$ be
%     \begin{equation}
%         \begin{aligned}
%             \mathcal{A}_t^i(x,u):=&\{j=1,\dots,m_{t}^i: [g_t^i(x_t,u_t)]_j=0\}, t\in\mathbf{I}_0^T, i\in\mathbf{I}_1^N\\
%             \mathcal{A}_{T+1}^i(x,u):=& \{j=1,\dots,m_{T+1}^i: [g_{T+1}^i(x_{T+1})]_j = 0\}, i\in\mathbf{I}_1^N
%         \end{aligned}
%     \end{equation}
%     where $[v]_j$ denotes the $j$-th entry of a vector $v$. We say the linear independence constraint qualification (LICQ) holds at $(x,u)$ if the vectors in the set
%     \begin{equation}
%         \cup_{i\in\mathbf{I}_1^N}\{\nabla_{x_t} h_t^i(x_t,u_t),\nabla_{u_t}h_t^i(x_t,u_t),\nabla_{x_t} g_t^i(x_t,u_t), \nabla_{u_t}g_t^i(x_t,u_t)\}
%     \end{equation}
%     are linearly independent for each $t\in\mathbf{I}_0^T$ and the vectors in the set $\{\nabla_{x_{T+1}} h_{T+1}^i(x_{T+1}),\allowbreak \nabla_{x_{T+1}} g_{T+1}^i(x_{T+1})\}$ are linearly independent as well. 
% \end{definition}
% Let $\mathcal{L}^i(x,u): = \sum_{t=0}^{T}\ell_t^i(x_t,u_t)+\ell_{T+1}(x_{T+1})$, for $i\in\{1,2\}$.
% {\color{red}Actually, we never used this assumption. We only require to have compact domain, and twice differentiable bounded objective function.}
% \begin{assumption}\label{assumption:monotone}
%     Each player's cost is twice differentiable. The function $F:\mathbb{R}^{(n+m)T}\to \mathbb{R}^{(Nn+m)T}$ defined by concatenating the gradient of each player's cost function, $F(\mathbf{x,u}):=\begin{bmatrix}\nabla_{\mathbf{[x,u]}} \mathcal{L}^i\end{bmatrix}_{i=1}^2$,
%     is a monotone operator, i.e., 
%     \begin{equation}
%         \begin{aligned}
%             \begin{bmatrix}
%                 \mathbf{x}-\tilde{\mathbf{x}}\\
%                 \mathbf{u}-\tilde{\mathbf{u}}
%             \end{bmatrix}^\top (F(\mathbf{x,u}) - F(\mathbf{\tilde{x},\tilde{u}})) \ge 0, \forall \mathbf{x}, \mathbf{\tilde{x}}\in\mathbb{R}^{nT},\mathbf{u},\tilde{\mathbf{u}}\in\mathbb{R}^{mT}
%             % \begin{bmatrix}
%             %     \nabla_{u_0^1} \ell_0^1(x_0,u_0^1,u_0^2)\\
%             %     \nabla_{u_0^2} \ell_0^2(x_0,u_0^1,u_0^2)\\
%             %     \nabla_{x_1} \ell_1^1(x_1,u_1^1,u_1^2) \\
%             %     \nabla_{x_1} \ell_1^2(x_1,u_1^1,u_1^)\\
%             %     \vdots\\
%             %     \nabla_{x_{T+1}} \ell_{T+1}^1(x_{T+1})\\
%             %     \nabla_{x_{T+1}} \ell_{T+1}^2(x_{T+1})
%             % \end{bmatrix}^\top \begin{bmatrix}\mathbf{u} - \tilde{\mathbf{u}} \\ \mathbf{x} - \tilde{\mathbf{x}} \end{bmatrix} \ge 0
%         \end{aligned}
%     \end{equation}
% \end{assumption}




We show in the following theorem that the dynamic programming problem can be rewritten as a sequence of nested constrained optimization problems, which encode the decision hierarchy of different players and also the impact of an action of a player to future stages.
\begin{theorem}\label{thm:nested constrained optimization problem}
    Consider an $N$-player feedback Stackelberg games. A set of strategies $\pi:=\{\pi_t^i\}_{t=0,i=1}^{T,N}$ constitutes a generalized feedback Stackelberg equilibrium if 
    % the leader's strategy satisfies
    % \begin{equation}\label{eq:leader's policy constrained problem}
    %     \begin{aligned}
    %         \pi_t^1(x_t) = \arg\min_{u_t^1 \in \mathcal{U}_t^{1*}} \   \|u_t^1\|_2^2 
    %     \end{aligned}
    % \end{equation}
    % where
    % \begin{equation}\label{eq:leader's constrained problem}
    %     \begin{aligned}
    %     \mathcal{U}_t^{1*}=\arg_{u_t^1} \min_{\substack{u_{t:T}^{1:N} 
    %     % \\ \tilde{u}_{t:T}^{2:N} 
    %     \\ x_{t+1:T+1}}} 
    %         &
    %         \sum_{\tau = t}^T \ell_\tau^1(x_\tau, u_\tau^{1:N}) + \ell_{T+1}^1 (x_{T+1})\\
    %         \textrm{s.t. }
    %         & 0 = u_\tau^j - \pi_\tau^j(x_\tau, u_\tau^{1:j-1} ) && \tau\in \mathbf{I}_{t}^T, j\in \mathbf{I}_{2}^N\\
    %         & 0=x_{\tau+1} - f_\tau(x_\tau, u_\tau^{1:N})&&\tau \in \mathbf{I}_{t}^T\\
    %         &0=h_\tau^1(x_\tau,u_\tau^{1:N})&&\tau \in \mathbf{I}_t^T\\
    %         & 0\le g_\tau^1(x_\tau, u_\tau^{1:N})&&\tau \in \mathbf{I}_t^T\\
    %         & 0 = h_{T+1}^1(x_{T+1})\\
    %         &0 \le g_{T+1}^1(x_{T+1})
    %     \end{aligned}
    % \end{equation}
    % \begin{equation}\label{eq:leader's policy constrained problem}
    %     \begin{aligned}
    %         \pi_t^1(x_t) = \arg\min_{\tilde{u}_t^1 \in \mathcal{U}_t^{1*}} \   \|\tilde{u}_t^1\|_2^2 
    %     \end{aligned}
    % \end{equation}
    % where
    % \begin{equation}\label{eq:leader's constrained problem}
    %     \begin{aligned}
    %     \mathcal{U}_t^{1*}=\arg_{u_t^1} \min_{\substack{u_{t:T}^1 \\ \tilde{u}_{t:T}^{2} \\ x_{t+1:T+1}}} 
    %         &
    %         \sum_{\tau = t}^T \ell_\tau^1(x_\tau, u_\tau^1, \tilde{u}_\tau^2) + \ell_{T+1}^1 (x_{T+1})\\
    %         \textrm{s.t. }
    %         & 0= \tilde{u}_\tau^j - \pi_\tau^j(x_\tau, u_\tau^{1:j-1}) && j\in \mathbf{I}_{i+1}^N,\tau\in \mathbf{I}_{t}^T \\
    %         & 0=x_{\tau+1} - f_\tau(x_\tau, u_\tau)&&\tau \in \mathbf{I}_{t}^T\\
    %         &0=h_\tau^1(x_\tau,u_\tau^1, \tilde{u}_\tau^{2})&&\tau \in \mathbf{I}_t^T\\
    %         & 0\le g_\tau^1(x_\tau, u_\tau^1, \tilde{u}_\tau^{2})&&\tau \in \mathbf{I}_t^T\\
    %         & 0 = h_{T+1}^1(x_{T+1})\\
    %         &0 \le g_{T+1}^1(x_{T+1})
    %     \end{aligned}
    % \end{equation}
    for all the players $i\in\{1,2,\dots,N\}$, at all $t\in \{0,1,\dots,T\}$, its strategy $\pi_t^i(x_t,u_t^{1:i-1})$ satisfies
    \begin{equation}\label{eq:player's policy constrained problem}
        \begin{aligned}
            \pi_t^i(x_t,u_t^{1:i-1}) = \arg \min_{u_t^i \in \mathcal{U}_t^{i*}}  \|u_t^i\|_2^2
        \end{aligned}
    \end{equation}
    where we define the best response set of player $i$ at time $t$ as
    \begin{subequations}\label{eq:player's constrained problem}
    \begin{align}
        \mathcal{U}_t^{i*}:= \arg_{u_t^i} \min_{\substack{
        u_{t}^{i:N} \\   u_{t+1:T}^{1:N}  \\ 
        x_{t+1:T+1}
        }} &\sum_{\tau = t}^T \ell_{\tau}^i(x_\tau, u_\tau)  +  \ell_{T+1}^i(x_{T+1})\\
        \textrm{s.t. }
        &0=u_{t}^j - \pi_t^{j}(x_t, u_t^{1:j-1}) && j\in  \mathbf{I}_{i+1}^N \label{eq:subsequent player's strategy} \\
        &0=u_{\tau}^j - \pi_\tau^{j}(x_\tau, u_\tau^{1:j-1}) && \tau \in \mathbf{I}_{t+1}^T,j\in\mathbf{I}_1^N\setminus\{i\} \label{eq:future player's strategy} \\
        % &0=u_{\tau}^j - \pi_\tau^{j}(x_\tau, u_\tau^{1:j-1}) && \tau \in \mathbf{I}_{t}^T,j\in \mathbf{I}_{i+1}^N \\
        &0=x_{\tau+1} - f_\tau(x_\tau,u_\tau) && \tau\in\mathbf{I}_{t}^T \\
        &0 = h_\tau^i(x_\tau,u_\tau) && \tau\in\mathbf{I}_{t}^T \\ 
        &0\le g_\tau^i(x_\tau,u_\tau) && \tau\in\mathbf{I}_{t}^T \\
        &0=h_{T+1}^i(x_{T+1})\\
        &0\le g_{T+1}^i(x_{T+1})
    \end{align}
    \end{subequations}
    where we drop \eqref{eq:subsequent player's strategy} when $i=N$, and we drop \eqref{eq:future player's strategy} when $t=T$. 
    % where $u_t^{1:i-1}=\emptyset$ when $i=1$ and $u_t^{i+1:N}=\emptyset$ when $i=N$. We also denote by $u_{t+1:T}^{1:i} = \emptyset$ when $t = T$.
\end{theorem}
\begin{proof}
% We approach the proof by showing that the optimal controls $\pi_t^{i*}$ defined in \eqref{eq:N-th player's strategy}, \eqref{eq:i-th player's strategy} and \eqref{eq:leader's strategy} are the same as 
% We approach the proof by showing that the set $\mathcal{U}_t^{i*}$ defined in \eqref{eq:N-th player's strategy}, \eqref{eq:i-th player's strategy} and \eqref{eq:leader's strategy}, for $i\in\mathbf{I}_1^N$, is equivalent to the set $\hat{\mathcal{U}}_t^{i*}$ in \eqref{eq:player's constrained problem}. 
% At the terminal time $t=T$, the $N$-th player's decision problem \eqref{eq:Z_t^N}
At the terminal time $t=T$, we observe that, for each player $i\in\mathbf{I}_1^N$, the set $\mathcal{U}_T^{i*}$ defined in \eqref{eq:player's constrained problem} can be rewritten as
\begin{align*}
    \mathcal{U}_T^{i*} =\arg_{u_T^i} \min_{u_T^i} \Bigg\{\min_{\substack{u_{T}^{i+1:N} \\ x_{T+1}}}&  \ell_{T}^i(x_T,u_T) + V_{T+1}^i(x_{T+1})\Bigg\}\\
    \textrm{s.t. }
    &0=u_{T}^j - \pi_T^{j}(x_T, u_T^{1:j-1}) && j\in  \mathbf{I}_{i+1}^N \\
    & 0=x_{T+1} - f_T(x_T,u_T) \\
    % &0 = u_T^j - \pi_T^j(x_T, u_T^{1:j-1}) && j\in\mathbf{I}_1^N\setminus \{i\} \\
    &0 = h_T^i(x_T,u_T),0\le g_T^i(x_T, u_T) \\
    & 0=h_{T+1}^i(x_{T+1}),0\le g_{T+1}^i(x_{T+1})
\end{align*}
which implies $\mathcal{U}_T^{i*}= \arg_{u_T^i} \min_{u_T^i} Z_T^i(x_T,u_T^{1:i-1},u_T^i)$
% \begin{align*}
%     \mathcal{U}_T^{i*}= \arg_{u_T^i} \min_{u_T^i} Z_T^i(x_T,u_T^{1:i-1},u_T^i)
%     % \mathcal{U}_T^{i*}= \arg_{u_T^i} \min_{\substack{
%     %         u_{T}^{i:N}  \\ 
%     %         x_{T+1}
%     %         }} & \ell_{T}^i(x_T, u^{1:N}_T)  +  \ell_{T+1}^i(x_{T+1})\\
%     %         \textrm{s.t. }
%     %         &0=u_{T}^j - \pi_T^{j}(x_T, u_T^{1:j-1}) && j\in  \mathbf{I}_{i+1}^N \\
%     %         &0=x_{T+1} - f_T(x_T,u_T^{1:N}) \\
%     %         &0 = h_T^i(x_T,u_T^{1:N})  ,0\le g_T^i(x_T,u_T^{1:N}) \\
%     %         &0=h_{T+1}^i(x_{T+1}),0\le g_{T+1}^i(x_{T+1})
% \end{align*}
and therefore $\pi_T^i = \pi_T^{i*}$. 
Moreover, for all $t\in \mathbf{I}_0^{T-1}$ and $i\in \mathbf{I}_1^N$, we observe
\begin{align*}
    \mathcal{U}_t^{i*}=\arg_{u_t^i} \min_{u_t^i} \Bigg\{\min_{\substack{u_{t:T}^{i+1:N} \\ x_{t+1:T+1}}}& \sum_{\tau = t}^T \ell_{\tau}^i(x_\tau,u_\tau) + \ell_{T+1}^i(x_{T+1})\Bigg\}\\
    \textrm{s.t. }
    & 0= u_t^j - \pi_t^j(x_t,u_t^{1:j-1}) && j\in \mathbf{I}_{i+1}^N \label{eq:}\\
    & 0=x_{\tau+1} - f_\tau(x_\tau,u_\tau) &&\tau\in\mathbf{I}_{t}^T \\
    &0 = u_\tau^j - \pi_\tau^j(x_\tau, u_\tau^{1:j-1}) && \tau\in \mathbf{I}_{t+1}^T,j\in\mathbf{I}_1^N\setminus \{i\} \\
    &0 = h_\tau^i(x_\tau,u_\tau) && \tau \in \mathbf{I}_{t}^T\\
    &0\le g_\tau^i(x_\tau, u_\tau) && \tau \in \mathbf{I}_t^T\\
    & 0=h_{T+1}^i(x_{T+1}) \\
    &0\le g_{T+1}^i(x_{T+1})
\end{align*}
% where we drop the first row when $i=N$. 
The above can be further rewritten as
\begin{align*}
    \mathcal{U}_t^{i*}=\arg_{u_t^i} \min_{u_t^i} \Bigg\{\min_{\substack{u_{t}^{i+1:N} \\ x_{t+1}}}&  \ell_{t}^i(x_t,u_t) + V_{t+1}^i(x_{t+1})\Bigg\}\\
    \textrm{s.t. }
    & 0= u_t^j - \pi_t^j(x_t,u_t^{1:j-1}) && j\in \mathbf{I}_{i+1}^N\\
    % & 0=u_{t+1}^j - \pi_{t+1}^j(x_{t+1}, u_{t+1}^{1:j-1}) && j \in \mathbf{I}_{1}^N\setminus \{i\}\\
    & 0=x_{t+1} - f_t(x_t,u_t) \\
    &0 = h_t^i(x_t,u_t) \\
    &0\le g_t^i(x_t, u_t)
\end{align*}
% which can be rewritten as
% \begin{align*}
%     V_t^i(x_t) = \min_{u_t^i} \min_{\substack{u_t^{i+1:N} \\ u_{t+1:T}^{1:N} \\ x_{t+1:T+1}}}
% \end{align*}
It follows that $\mathcal{U}_T^{i*} = \arg_{u_t^i} \min_{u_t^i} Z_t^i(x_t,u_t^{1:i-1},u_t^i)$, 
% \begin{equation}
%     \mathcal{U}_T^{i*} = \arg_{u_t^i} \min_{u_t^i} Z_t^i(x_t,u_t^{1:i-1},u_t^i)
% \end{equation}
which implies $\pi_t^i = \pi_t^{i*}$. 
% \begin{align*}
%     \mathcal{U}_t^{i*}= \arg_{u_t^i} \min_{\substack{u_{t}^{i:N} \\ x_{t+1}}} \ &  \begin{aligned}\ell_t^i(x_t,u_t^{1:N}) + \min_{\substack{ u_{t+1:T}^{1:N}  \\ x_{t+2:T+1} }} & \sum_{\tau = t+1}^T \ell_{\tau}^i(x_\tau, u^{1:N}_\tau)  +  \ell_{T+1}^i(x_{T+1})\\
%     \textrm{s.t. }&0=u_{\tau}^j - \pi_\tau^{j}(x_\tau, u_\tau^{1:j-1}), \tau \in \mathbf{I}_{t+1}^T,j\in \mathbf{I}_1^N\setminus\{i\} \\
%     &0=x_{\tau+1} - f_\tau(x_\tau,u_\tau^{1:N}) , \tau\in\mathbf{I}_{t}^T \\
%     &0 = h_\tau^i(x_\tau,u_\tau^{1:N}) , \tau\in\mathbf{I}_{t}^T \\ 
%     &0\le g_\tau^i(x_\tau,u_\tau^{1:N}) , \tau\in\mathbf{I}_{t}^T \\
%     &0=h_{T+1}^i(x_{T+1})\\
%     &0\le g_{T+1}^i(x_{T+1})\end{aligned}\\
%     \textrm{s.t. }&0=u_{t}^j - \pi_t^{j}(x_t, u_t^{1:j-1}),j\in  \mathbf{I}_{i+1}^N && \\
%     &0=x_{t+1} - f_t(x_t,u_t^{1:N}) 
% \end{align*}
% \eqref{eq:N-th player's strategy}, \eqref{eq:i-th player's strategy} and \eqref{eq:leader's strategy} can be rewritten as
% We approach the proof by backward induction. For a time $t\in\mathbf{I}_0^T$, by definition of $\pi_t^i$ in \eqref{eq:player's constrained problem}, there exists an $\epsilon>0$ such that player $i$'s state-action function satisfies
% \begin{equation}
%     \begin{aligned}
%         Z_t^i(x_t,u_t^{1:i-1},\tilde{u}_t^i)\ge Z_t^i(x_t,u_t^{1:i-1},\pi_t^i(x_t,u_t^{1:i-1})), 
%     \end{aligned}
% \end{equation}
% for all $\tilde{u}_t^i \in \{u_t^i:\|u_t^i - \pi_t^i(x_t,u_t^{1:i-1})\|\le \epsilon\}$. Observe that we can rewrite $Z_t^i(x_t,u_t^{1:i})$ by introducing the control strategy constraints $0=u_t^j - \pi_t^j(x_t,u_t^{1:j-1})$, $j\in \mathbf{I}_{i+1}^N$, and $0=u_\tau^j -\pi_\tau^j(x_\tau, u^{1:j-1}) $, for $\tau\in\mathbf{I}_{t+1}^T$, $j\in \mathbf{I}_{1}^{i-1}\cup \mathbf{I}_{i+1}^N$,
% \begin{equation}
%         Z_t^i(x_t,u_t^{1:i}) = \left\{ \begin{aligned}&\ell_t^i(x_t,u_t^{1:N})+V_{t+1}^i(x_{t+1})
%         && \textrm{if } \left\{\begin{aligned}\substack{  u_t^j = \pi_t^j(x_t,u_t^{1:j-1}),j\in\mathbf{I}_{i+1}^N\\ 
%         x_{t+1} = f_t(x_t,u_t^{1:N})\\
%         % 0= h^i_{T+1}(x_{T+1}) \\ 
%         0 = h^i_t(x_t,u_t^{1:N}) \\ 
%         % 0\le g^i_{T+1}(x_{T+1})\\
%         0 \le g^i_t(x_t,u_t^{1:N})
%         }
%         \end{aligned}\right.\\
%         & \infty && \textrm{otherwise} \end{aligned}\right.
% \end{equation}
% % Recall that $V_{t+1}^i(x_{t+1})$ is defined as
% % \begin{equation}
% %     \begin{aligned}
% %         V_{t+1}^i(x_{t+1}) = \min 
% %     \end{aligned}
% % \end{equation}
% By definition of $\pi_T^i$, there exists $\epsilon>0$ such that
% \begin{equation}
%     \begin{aligned}
%         Z_T^1(x_T,u_T^1)\ge Z_T^1(x_T, \pi_t^1(x_T)),\ \forall u_t^1\in\{u_t^1:\|u_t^1 - \pi_t^1(x_t)\|_2^2\le \epsilon\}
%     \end{aligned}
% \end{equation}
% For the cases when $t<T$, we can rewrite the follower's decision problem as 
% \begin{equation}
%         Z_t^2(x_t,u_t^1,u_t^2) = \left\{ \begin{aligned} &   \ell_t^2(x_t,u_t^2,u_t^2) +     && \textrm{if }\left\{ \substack{
%         x_{t+1} = f_t(x_t,u_t^{1:N})\\
%         u_T^2 = \pi_T^2(x_T, u_T^{1:N})
%         } \right. \\ & \infty  && \textrm{otherwise} \end{aligned} \right.
% \end{equation}
% and there exists $\epsilon>0$ such that
% \begin{equation}
% \begin{aligned}    
%     Z_t^2(x_t,u_t^1,u_t^2) &\ge Z_t^2(x_t,u_t^1, \pi_t^2(x_t,u_t^1)),\ \forall u_t^2 \in \{u_t^2:\|u_t^2-\pi_t^2(x_t,u_t^1)\|_2^2\le \epsilon\}\\
%     Z_t^1(x_t,u_t^1)& \ge Z_t^1(x_t,\pi_t^1(x_t)),\ \forall u_t^1\in \{u_t^1:\|u_t^1 - \pi_t^1(x_t)\|_2^2\le \epsilon\}
% \end{aligned}
% \end{equation}
Therefore, the set of strategies $\{\pi_t^i\}_{t=0,i=1}^{T,N}$ constitutes a generalized feedback Stackelberg equlibrium strategy.
\end{proof}
% How can you show that the map from state to control is a continuous or even differentiable map?







%     \begin{equation}
%         \begin{aligned}
%             \pi_t^2(x_t,u_t^1): = \tilde{u}_t^2\in \arg_{u_t^2} \min_{\substack{u_{t:T}^2 \\ \tilde{u}_{t+1:T}^{1} \\ x_{t+1:T+1}}} 
%             &\sum_{\tau = t}^T \ell_\tau^2(x_\tau, \tilde{u}_\tau^1, u_\tau^2) + \ell_{T+1}^2 (x_{T+1})\\
%             \textrm{s.t. }& 0 = \tilde{u}_\tau^{1} - \pi_\tau^{1}(x_\tau) &&\tau \in \{t+1,\dots,T\}\\
%             & 0=x_{\tau+1} - f_\tau(x_\tau, \tilde{u}_\tau^1, u_\tau^{2})&&\tau \in \{t,\dots,T\}\\
%             & 0=h_\tau^2(x_\tau,\tilde{u}_\tau^1, u_\tau^{2})&&\tau \in \{t,\dots,T\}\\
%             & 0\le g_\tau^2(x_\tau, \tilde{u}_\tau^1, u_\tau^{2})&&\tau \in \{t,\dots,T\}\\
%             & 0 = h_{T+1}^2(x_{T+1})\\
%             &0 \le g_{T+1}^2(x_{T+1})
%         \end{aligned}\label{eq:GFSB equation2}
%     \end{equation}
%     and for other players
%     \begin{equation}
%         \begin{aligned}
%             \pi_t^3(x_t,u_t^1,u_t^2):= \tilde{u}_t^3 \in \arg_{u_t^2} \min_{u_{t,T}^3} & \sum_{\tau=t}^T \ell_\tau^3(x_\tau,u_\tau) + \ell_{T+1}^3(x_{T+1})\\
%             \textrm{s.t. }&0=
%         \end{aligned}
%     \end{equation}

% \begin{equation}
%     V_{t}^1(x_t):= \left\{ \begin{aligned}
%         &\ell_{t}^1(x_t,u_t^1, u_t^2)+ V_{t+1}^1(x_{t+1}) &&\textrm{if }h_{t}^1(x_{t}, u_t^1,u_t^2)=0,\ g_t^1(x_t,u_t^1,u_t^2)\ge 0\\
%         & \infty && \textrm{else.}
%     \end{aligned} \right.
% \end{equation}
% and
% \begin{equation}
%     V_t^2(x_t):= \left\{ \begin{aligned}
%         & \ell_t^2(x_t,u_t^1,u_t^2)+V_{t+1}^2(x_{t+1}) && \textrm{if }h_t^2(x_t,u_t^1,u_t^2)=0,\ g_t^2(x_t,u_t^1,u_t^2)\ge 0\\ &\infty && \textrm{else.} 
%     \end{aligned} \right. 
% \end{equation}
In what follows, we will characterize the KKT conditions of the constrained optimization problems in \eqref{eq:player's constrained problem}. Before we doing that, we first introduce Lagrange multipliers, which facilitates the formulation of Lagrangian function, and therefore paves the way for KKT conditions. %Before doing that, we introduce a few assumptions to facilitate the discussion.



% {\color{red}Note that even though we have this monotone gradient assumption, how can we say that the log penalty will not destroy this assumption if we don't have convex feasible domain? }


% \begin{assumption}
%     The gradient vector $[\nabla_{x_t}\ell_t^1, \nabla_{u_t^1}\ell_t^1, \nabla_{x_t}\ell_t^2, \nabla_{u_t^2}\ell_t^2]$ is a strongly monotone operator.
% \end{assumption}

% {\color{red}Show the differentiability of the policy?}
% So, we know that if there exits a solution to the optimization problem at each stage, then from the definition of policy, we want to show that
% \begin{equation}
%     \lim_{\tilde{x}\to x}\frac{\partial u^*(\tilde{x})}{\partial \tilde{x}}
% \end{equation}
% exists. Essentially, that requires to have the existence of the solution.
% \begin{remark}\color{red}
%     Is it true that we will lose differentiability of the policy when having binding constraints? What about if we show that the policy resulted from PDIP will be differentiable? Yeah, that's true. So, a good solution can be that proving that the strategies derived from the log-penalized objectives are differentiable. 
% \end{remark}

% \begin{enumerate}\color{red}
%     \item Even though we have the above assumption, the problem of the convergence proof is still, we don't know what an optimal strategy looks like. The difficulty comes from that the higher order gradient term of the policy is hard to compute. So, that motivates the quasi-Newton approximation. 
%     \item What about we show that the algorithm converges to the Quasi-Newton optimal solution?
% \end{enumerate}

Let $t\in\mathbf{I}_0^{T}$ and $i\in\mathbf{I}_1^N$. We denote by $\lambda_t^i\in\mathbb{R}^{n}$ the Lagrange multiplier for the dynamics constraint $0=x_{t+1}-f_t(x_t,u_t)$. We also define $\mu_t^i\in\mathbb{R}^{l_{h,t}^i}$ and $\gamma_t^i\in\mathbb{R}^{l_{g,t}^i}$ to be the Lagrange multipliers for the constraints $0=h_t^i(x_t,u_t)$ and $0\le g_t^i(x_t,u_t)$, respectively. In particular, when $t\le T$, the constrained problem \eqref{eq:player's constrained problem} of player $i<N$ considers the feedback interaction constraint $0=u_t^j - \pi_t^j(x_t,u_t^{1:j-1})$, $j\in\mathbf{I}_{i+1}^N$. Thus, we associate those constraints with multipliers $\psi_t^i:=[\psi_t^{i,i+1},\psi_t^{i,i+2},\dots,\psi_t^{i,N}]$, where $\psi_t^{i,j}\in\mathbb{R}^{m_i}$. Moreover, when $t<T$, the constrained problem \eqref{eq:player's constrained problem} of a player $i\le N$ includes the feedback interaction constraints $0=u_{t+1}^j -\pi_{t+1}^j(x_{t+1},u_{t+1}^{1:j-1}) $, for $j\in \mathbf{I}_1^N\setminus\{i\}$. Thus, we associate those constraints with multipliers $\eta_t^i:=[\eta_t^{i,1},\dots, \eta_t^{i,i-1}, \eta_t^{i,i+1},\allowbreak\dots,\eta_t^{i,N}]$, where $\eta_t^{i,j}\in\mathbb{R}^{m_j}$. Finally, we simplify the notation by defining $\lambda_t:=[\lambda_t^1,\lambda_t^2,\dots,\lambda_t^N]$, and define $\mu_t$, $\gamma_t$, $\eta_t$, and $\psi_t$ accordingly.  

In what follows, we define the Lagrangian functions of all the players. We first consider the player $i\in \mathbf{I}_{1}^{N-1}$, 
% \begin{equation}
%     \begin{aligned}
%         L_t^1(x_t,&x_{t+1},u_t,u_{t+1} \lambda_t, \mu_t, \gamma_t, \eta_t, \psi_t): =  \ell_{t}^1(x_t,u_t)+\lambda_t^{1\top} (x_{t+1}-f_t(x_t,u_t)) \\
%         &- \mu_t^{1\top} h_t^1(x_t,u_t)-\gamma_t^{1\top} g_t^1(x_t,u_t) \\& + \sum_{j\in\mathbf{I}_2^N} \psi_t^{1,j^\top} (u_t^j - \pi_t^j(x_t,u_t^{1:j-1})) %+\psi_t^{1,2\top} (u_t^2 - \pi_t^2(x_t,u_t^{1}))  +\dots + \psi_t^{1,N\top} (u_t^N - \pi_t^N(x_t,u_t^{1:N-1})) 
%          + \sum_{j\in\mathbf{I}_2^N} \eta_t^{1,j\top} (u_{t+1}^j - \pi_{t+1}^j(x_{t+1},u_{t+1}^{1:j-1}))  %\eta_t^{1,2\top}(u_{t+1}^{2} - \pi_{t+1}^2(x_{t+1},u_{t+1}^{1}))
%         %+\dots+ \eta_t^{1,N\top} (u_{t+1}^N - \pi_{t+1}^N(x_{t+1},u_{t+1}^{1:N-1}))  
%     \end{aligned}
% \end{equation}
% where the terms represent the player $i$'s cost, dynamics constraint, equality and inequality constraint, and constraints encoding the feedback interaction among players at the current and next time steps. 
% Similarly, for the player $i\in\{2,\dots,N-1\}$, we have
\begin{equation}\label{eq:Lagrangian for other players, time t}
    \begin{aligned}
        L_t^i(x_{t:t+1},u_{t:t+1},\lambda_t,\mu_t, \gamma_t, \eta_t,\psi_t): =& \ell_{t}^i(x_t,u_t) + \lambda_t^{i\top} (x_{t+1} - f_t(x_t,u_t)) \\
        &- \mu_t^{i\top } h_t^i(x_t,u_t)-\gamma_t^{i\top }g_t^i(x_t,u_t) \\ & + \sum_{j\in\mathbf{I}_{i+1}^N} \psi_t^{i,j\top}(u_t^{j} - \pi_t^j(x_t,u_t^{1:j-1})) %\psi_{t}^{i,i+1\top}(u_{t}^{i+1} - \pi_{t}^{i+1}(x_t,u_t^{1:i+1}))
         %+ \dots + \psi_{t}^{i,N\top}(u_t^N - \pi_t^N(x_t,u_t^{1:N-1})) 
          \\&+ \sum_{j\in \mathbf{I}_1^N\setminus\{i\}}  \eta_t^{i,j^\top} (u_{t+1}^j - \pi_{t+1}^j(x_{t+1}, u_{t+1}^{1:j-1})) %  + \eta_t^{i,1\top} (u_{t+1}^1 - \pi_{t+1}^1(x_t) )+\dots+\eta_{t}^{i,i-1\top}(u_{t+1}^{i-1} - \pi_{t+1}^{i-1}(x_{t+1},u_{t+1}^{1:i-1}))+\dots  \\ & + \eta_{t}^{i,i+1\top}(u_{t+1}^{i+1} - \pi_{t+1}^{i+1}(x_{t+1},u_{t+1}^{1:i+1})) + \dots  +\eta_{t}^{i,N\top}(u_{t+1}^N - \pi_{t+1}^N(x_{t+1},u_{t+1}^{1:N-1}))
    \end{aligned}
\end{equation}
where the right handside terms represent the player $i$'s cost, dynamics constraint, equality and inequality constraints, and constraints encoding the feedback interaction among players at the current and next time steps. Similarly, for the player $N$, we consider
\begin{equation}\label{eq:Lagrangian for leader, time t}
    \begin{aligned}
        L_t^N(x_{t:t+1},u_{t:t+1},\lambda_t,\mu_t, \gamma_t, \eta_t,\psi_t): =& \ell_{t}^N(x_t,u_t) + \lambda_t^{N\top} (x_{t+1} - f_t(x_t,u_t)) \\
        &- \mu_t^{N\top } h_t^N(x_t,u_t)-\gamma_t^{N\top }g_t^N(x_t,u_t) \\ & +  \sum_{j\in\mathbf{I}_{1}^{N-1}} \eta_t^{N,j\top} (u_{t+1}^j - \pi_{t+1}^j(x_{t+1}, u_{t+1}^{1:j-1}))  % \eta_t^{N,1\top} (u_{t+1}^1 - \pi_{t+1}^1(x_t) ) + \dots   + \eta_{t}^{N,N-1\top} (u_{t+1}^{N-1} - \pi_{t+1}^{N-1}(x_{t+1},u_{t+1}^{1:N-1}))
    \end{aligned}
\end{equation}
where the right handside terms represent the player $N$'s cost, dynamics constraint, equality and inequality constraints, and constraints encoding the feedback interaction among players at next time step. Notice that we don't consider the feedback interaction among players at the current step in \eqref{eq:Lagrangian for leader, time t} because player $N$ is the last player making decision at the stage $t$. This is the major difference between \eqref{eq:Lagrangian for leader, time t} and \eqref{eq:Lagrangian for other players, time t}.
% \begin{equation}
%     \begin{aligned}
%     L_t^2(x_t,u_t,\lambda_t, \mu_t, \gamma_t, \eta_t, \psi_t^1) := &\ell_t^2(x_t,u_t) + \lambda_t^{2\top} (x_{t+1} - f_t(x_t,u_t)) - \mu_t^{2\top} h_t^2(x_t,u_t) \\ & - \gamma_t^{2\top}g_t^2(x_t,u_t)+ \eta_t^{2\top} (u_{t+1}^1 - \pi_{t+1}^1(x_{t+1})) \\
% L_t^1(x_t,u_t,\lambda_t,\mu_t,\gamma_t, \eta_t, \psi_t^1):= & \ell_t^1(x_t,u_t) + \lambda_t^{1\top} (x_{t+1} - f(x_t,u_t)) - \mu_t^{1\top} h_t^1(x_t,u_t) \\ & - \gamma_t^{1\top} g_t^1(x_t,u_t) + \eta_t^{1\top}(u_{t+1}^2 - \pi_{t+1}^2(x_{t+1},u_{t+1}^1))\\ %\hat{\pi}_{t+1}^2(x_t) - \check{\pi}_{t+1}^2(u_{t+1}^1)) \\ 
% &+\psi_t^{1\top}(u_t^2 - \pi_{t}^2(x_t,u_t^1))
%     \end{aligned}
% \end{equation}

Furthermore, at the terminal time $t=T$, for player $i\in\mathbf{I}_1^{N-1}$, we consider
% \begin{equation}
%     \begin{aligned}
%     L_{T}^1(x_T,&x_{T+1},u_T,\lambda_T, \mu_T, \gamma_T ,\psi_T,\gamma_{T+1},\mu_{T+1}):=\ell_T^1(x_T,u_T) + \ell_{T+1}^1(x_{T+1}) \\& + \lambda_T^{1\top}(x_{T+1} - f_T(x_T,u_T)) - \mu_T^{1\top}h_T^1(x_T,u_T) - \gamma_T^{1\top}g_T^1(x_T,u_T)\\ & -\gamma_{T+1}^{1\top} g_{T+1}^1(x_{T+1})  - \mu_{T+1}^{1\top} h_{T+1}^1(x_{T+1}) + \psi_{T}^{1,2\top}(u_T^2 - \pi_T^2(x_T,u_T^1))\\
%     & + \dots + \psi_T^{1,N^\top}(u_T^N - \pi_T^N(x_T,u_T^{1:N-1}))
%     \end{aligned}
% \end{equation}
% for the player $i\in \{2,\dots,N-1\}$,
\begin{equation}\label{eq:Lagrangian of player i, time T}
    \begin{aligned}
        L_{T}^i(x_{T:T+1},u_T,\lambda_T, \mu_{T:T+1}, \gamma_{T:T+1} ,\psi_T):=&\ell_T^i(x_T,u_T) + \ell_{T+1}^i(x_T) \\& + \lambda_T^{i\top} (x_{T+1} - f_T(x_T,u_T)) \\ & - \mu_T^{i\top}h_T^i(x_T,u_T) - \mu_{T+1}^{i\top} h_{T+1}^i(x_{T+1}) \\& - \gamma_T^{i\top}g_T^i(x_T,u_T)-\gamma_{T+1}^{i\top} g_{T+1}^i(x_{T+1})   \\ & + \sum_{j\in \mathbf{I}_{i+1}^N} \psi_T^{i,j\top} (u_T^j - \pi_T^j(x_T,u_T^{1:j-1})) % + \psi_{T}^{i,i+1\top}(u_T^{i+1} - \pi_T^{i+1}(x_T, u_T^{1:i}))\\
    % & + \dots + \psi_T^{i,N^\top}(u_T^N - \pi_T^N(x_T,u_T^{1:N-1}))
    \end{aligned}
\end{equation}
where the right handside terms represent the player $i$'s costs, dynamics constraint, equality and inequality constraints, and constraints encoding the feedback interaction among players at the terminal time $T$. Note that there is no more decision to be made at the time $t=T+1$, and therefore, there is no term representing the feedback interactions among players for future time steps in \eqref{eq:Lagrangian of player i, time T}, which is different from \eqref{eq:Lagrangian for other players, time t} and \eqref{eq:Lagrangian for leader, time t}. 

Finally, for the $N$-th player, we have
\begin{equation}\label{eq:Lagrangian of leader, time T}
    \begin{aligned}
        L_{T}^N(x_{T:T+1},u_T,\lambda_T, \mu_{T:T+1}, \gamma_{T:T+1} ,\psi_T):=&\ell_T^N(x_T,u_T) + \ell_{T+1}^N(x_T) \\& + \lambda_T^{N\top} (x_{T+1} - f_T(x_T,u_T)) \\ & - \mu_T^{N\top}h_T^N(x_T,u_T)  - \mu_{T+1}^{N\top} h_{T+1}^N(x_{T+1}) \\&  - \gamma_T^{N\top}g_T^N(x_T,u_T)  -\gamma_{T+1}^{N\top} g_{T+1}^N(x_{T+1}) 
    \end{aligned}
\end{equation}
where the right handside terms represent that player $N$'s costs, dynamics constraint, equality and inequality constraints. Since player $N$ is the last player that makes decision, we don't account for any feedback interaction among players, which is different from \eqref{eq:Lagrangian of player i, time T}.

%Combining \eqref{eq:Lagrangian for other players, time t}, \eqref{eq:Lagrangian for leader, time t}, \eqref{eq:Lagrangian of player i, time T} and \eqref{eq:Lagrangian of leader, time T}, 
For all the time steps $t\in\mathbf{I}_0^T$ and players $i\in\mathbf{I}_1^N$, assuming the state $x_t$ is given and players in front of $i$, if exists, have all taken actions, i.e., player $j\in\mathbf{I}_1^{i-1}$ takes $u_t^j$, we formulate the Lagrangian of the problem \eqref{eq:player's constrained problem} of player $i$ at the $t$-th stage as
\begin{equation}
    \begin{aligned}    
        \mathcal{L}_t^i (&x_{t:T+1}, u_{t:T}, \lambda_{t:T}, \mu_{t:T+1}, \gamma_{t:T+1}, \eta_{t:T-1},\psi_{t:T} ): = \sum_{\tau=t}^{T-1} L_\tau^i(x_{\tau:\tau+1},u_{\tau:\tau+1}, \\ &\lambda_\tau, \mu_\tau, \gamma_\tau, \eta_\tau, \psi_\tau)  + L_T^i(x_{T:T+1},u_T,\lambda_T, \mu_{T:T+1}, \gamma_{T:T+1}, \psi_T)
    \end{aligned}
\end{equation}
In what follows, we will propose KKT condition for the nested constrained optimization problem \eqref{eq:player's constrained problem}. We concatenate the KKT conditions of each player at each time step, and we summarize the overall KKT conditions in the following theorem.
\begin{theorem}[Necessary Condition]\label{thm:necessary condition}
    The KKT condition of \eqref{eq:player's constrained problem} can be formulated as 
    \begin{equation}\label{eq:KKT}
        \begin{aligned}
            0&\in\nabla_{u_{t}^i}\mathcal{L}_t^i (x_{t:T+1}, u_{t:T}, \lambda_{t:T}, \mu_{t:T+1}, \gamma_{t:T+1}, \eta_{t:T-1},\psi_{t:T} )\\
            0&\in\nabla_{x_{\tau}} \mathcal{L}_t^i (x_{t:T+1}, u_{t:T}, \lambda_{t:T}, \mu_{t:T+1}, \gamma_{t:T+1}, \eta_{t:T-1},\psi_{t:T} ), &&\tau \in \mathbf{I}_{t+1}^{T+1}\\
            0&\in\nabla_{u_{t}^{j}}\mathcal{L}_t^i (x_{t:T+1}, u_{t:T}, \lambda_{t:T}, \mu_{t:T+1}, \gamma_{t:T+1}, \eta_{t:T-1},\psi_{t:T} ),&& j\in \mathbf{I}_{i+1}^N\\%, \tau' \in \mathbf{I}_{t}^T \\
            0&\in\nabla_{u_{\tau}^{j}}\mathcal{L}_t^i (x_{t:T+1}, u_{t:T}, \lambda_{t:T}, \mu_{t:T+1}, \gamma_{t:T+1}, \eta_{t:T-1},\psi_{t:T} ),&& j\in\mathbf{I}_{1}^N\setminus\{i\}, \tau\in \mathbf{I}_{t+1}^T\\
            0& = x_{\tau+1} - f_\tau(x_\tau,u_\tau), && \tau\in \mathbf{I}_{t}^T\\
            0&=h_\tau^i(x_\tau,u_\tau), && \tau\in \mathbf{I}_{t}^T\\ 
            0&\le \gamma_\tau^{i} \perp g_\tau^i(x_\tau,u_\tau)\ge 0, && \tau\in \mathbf{I}_{t}^T\\
            0&= h_{T+1}^i(x_{T+1}),\\
            0&\le \gamma_{T+1}^{i} \perp g_{T+1}^i(x_{T+1})\ge 0
\end{aligned}
    \end{equation}
    where $i\in\mathbf{I}_1^N$ and $t\in\mathbf{I}_0^T$. We define $x: = [x_t]_{t=0}^{T+1}$, $u:=[u_t]_{t=0}^T$, $\lambda:=[\lambda_t]_{t=0}^T$, $\mu:=[\mu_t]_{t=0}^T$, $\gamma: = [\gamma_t]_{t=0}^T$, $\eta: = [\eta_t]_{t=0}^{T-1}$, and $\psi:=[\psi_t]_{t=0}^T$. 
    Under Assumption~\ref{assumption:feasible}, there exists Lagrange multipliers $\{\lambda,\mu,\gamma,\eta,\psi\}$ and state and control trajectories $\{x,u\}$ along with strategies $\{\pi_t^i\}_{t=0,i=1}^{T,N}$ such that \eqref{eq:KKT} holds true.
\end{theorem}
\begin{proof}
    For a time $t\in\mathbf{I}_0^T$ and player $i\in\mathbf{I}_1^N$, we set the gradient of $\mathcal{L}_t^i$ with respect to $u_t^i$ and $x_t$ to be zero. This constitutes the first two rows of \eqref{eq:KKT}. In addition, a player $i<N$ considers the feedback interaction constraints $0=u_t^j - \pi_t^j(x_t,u_1^{j-1})$, for $j\in\mathbf{I}_{i+1}^N$. Thus, we need to set the gradient of $\mathcal{L}_t^i$ with respect to $u_t^j$ to be zero, for $j\in\mathbf{I}_{i+1}^N$. This is the third row of \eqref{eq:KKT}. Moreover, at a time $t<T$, each player $i\in \mathbf{I}_1^N$ needs to account for the feedback reaction from other players at the next step. We set the gradient of $\mathcal{L}_t^i$ with respect to $u_t^j$ to be zero, where $j\in\mathbf{I}_1^N\setminus \{i\}$. Finally, we include the dynamcis constraints, equality and inequality constraints, and complementary slackness conditions in the last three rows of \eqref{eq:KKT}.
\end{proof}
\begin{remark}
    Note that we don't explicitly ensure the control policy constraint $u_t^{j} = \pi_t^{j}(x_t,u_t^{1:j-1}) $, $j\in \mathbf{I}_1^N\setminus \{i\}$, because it is implicitly ensured by the first-order optimality condition for $u_t^j$.
\end{remark}

% \begin{remark}
%     However, 
% \end{remark}
% {\color{blue}\begin{remark}
%     You may want to argue that we apply Newton method and therefore the integration lemma follows immediately though we have variational inequality problem here. It may be worthwhile to check papers about applying Newton's method to variational inequality problems. 
% \end{remark}}
% We will drop the rows of the KKT conditions if those rows are not linear independent to the other rows.\\ 

\begin{theorem}[Sufficient Condition]\label{thm:sufficient condition}
    Suppose $\{x,u,\lambda, \mu, \gamma, \eta, \psi\}$ and its associated strategy set $\{\pi_t^i\}_{t=0,i=1}^{T,N}$ satisfy \eqref{eq:KKT} and there exists an $\epsilon>0$ such that the following condition holds true, for all $t\in \{0,1,\dots,T\}$
    \begin{equation}\label{eq:sufficient condition}
        \begin{aligned}
            &\sum_{\tau=t}^T \begin{bmatrix}
                \Delta x_\tau \\ \Delta u_\tau
            \end{bmatrix}^\top \nabla^2_{[x_\tau,u_\tau]} L_\tau^{i}\begin{bmatrix}
                \Delta x_\tau \\ \Delta u_\tau
            \end{bmatrix} + \Delta x_{T+1}^\top \nabla^2_{x_{T+1}} L_{T+1}^i\Delta x_{T+1}>0\\
            & \forall \{\Delta x_{T+1}\}\cup\{\Delta x_\tau, \Delta u_\tau\}_{\tau=t}^T:  \\
            % &\hspace{2cm} 0= \Delta u_{\tau}^i - \nabla_{[x_t,u_]} \pi_\tau^i (x_\tau)\Delta x_\tau,\tau \in \mathbf{I}_{t}^T\\
            % &\hspace{4cm} 0=\Delta u_\tau^2 - \begin{bmatrix}
            %     \nabla_x \pi_\tau^2(x_\tau, u_\tau^1) \\ \nabla_{u^1} \pi_\tau^2(x_\tau, u_\tau^1)
            % \end{bmatrix}^\top \begin{bmatrix}
            %    \Delta  x_\tau\\ \Delta u^1_\tau
            % \end{bmatrix}\\
            &\hspace{2cm} 0=\Delta u_t^j - \nabla_{[x_t,u_t^{1:j-1}]} \pi_t^i(x_t,u_t^{1:j-1})\begin{bmatrix}\Delta x_t \\ \Delta u_t^{1:j-1} \end{bmatrix},j\in \mathbf{I}_{i}^N\\
            &\hspace{2cm} 0=\Delta u_\tau^j - \nabla_{[x_\tau,u_\tau^{1:j-1}]} \pi_\tau^i(x_\tau,u_\tau^{1:j-1})\begin{bmatrix}\Delta x_\tau \\ \Delta u_\tau^{1:j-1} \end{bmatrix},j\in \mathbf{I}_{1}^N,\tau\in\mathbf{I}_{t+1}^T\\
            &\hspace{2cm} 0= \Delta x_{\tau+1} - \nabla_{[x_\tau,u_\tau]} f_\tau(x_\tau, u_\tau) \begin{bmatrix}
                \Delta x_{\tau} \\ \Delta u_\tau 
            \end{bmatrix},\tau\in \mathbf{I}_{t}^T 
            % \\
            % &\hspace{2cm} 0<\|\Delta x_\tau\|_2\le \epsilon,  0<\|\Delta u_\tau\|_2\le \epsilon, \tau \in \mathbf{I}_{t}^T\\
            % &\hspace{2cm} 0<\|\Delta x_{T+1}\|_2\le \epsilon
            % &\hspace{2cm} 0=\Delta u_\tau^{2}  - \nabla_x \pi_\tau^{2}(x_\tau,u_\tau^1) \Delta x_\tau - \nabla_{u_\tau^1}\pi_\tau,\ \textrm{if }i=1\\
            % &\hspace{2cm} 0 = \Delta u_\tau^2 - \nabla_1,\ \textrm{if }i=2
        \end{aligned}
    \end{equation}
    then, $\{\pi_t^i\}_{t=0,i=1}^{T,2}$ is a local generalized feedback Stackelberg equilibrium.
\end{theorem}
\begin{proof}
    We can check that the feasible set to the equality constraints of \eqref{eq:sufficient condition} is a superset of the critical cone of the problem \eqref{eq:KKT}. By Theorem 12.6 in \cite{nocedal1999numerical}, the solutions $(\mathbf{x},\mathbf{u})$ constitute a local generalized feedback Stackelberg equilibrium trajectory, and the strategies $\{\pi_t^i\}_{t=0,i=1}^{T,N}$ are generalized feedback Stackelberg equilibrium. 
\end{proof}

Theorems~\ref{thm:necessary condition} and \ref{thm:sufficient condition} establish condition to certify whether a given sequence of strategies $\{\pi_t^i\}_{t=0,i=1}^{T,N}$ and the trajectory under it constitute a feedback Stackelberg equilibrium. When we don't have those given strategies $\{\pi_t^i\}_{t=0,i=1}^{T,N}$, the computation of them is not trivial. In the following sections, we will discuss how to compute those strategies. We will first compute feedback strategies for Linear Quadratic games and then extend the result to nonlinear games. 

% {\color{red}
% Suppose the ground truth GFSE strategy is $\pi_t^{i*}$, then there exists a Quasi policy approximation $\tilde{\pi}_t^i$ that satisfies the KKT condition. 
% \begin{equation}
%     \begin{aligned}
%         \tilde{\pi}_t^i(x_t,u_t^{1:i-1}): = u_t^* - \nabla \pi_t^{i*}(x_t^*,u_t^{1:i-1*}) \begin{bmatrix}
%              x_t - x_t^* \\ u_t^{1:i-1} - u_t^{1:i-1*}
%         \end{bmatrix}
%     \end{aligned}
% \end{equation}
% }

% \begin{proposition}
%     Suppose that the KKT Jacobian $\nabla K$ has full rank, and the dynamics is $L$-Lipschitz continuous, then 
%     \begin{equation}
%         \begin{aligned}
%             \|u_t - u_t^* \| \le \mathcal{O}(LNT\|K\|)
%         \end{aligned}
%     \end{equation}
%     then, this is not an optimal solution when we apply Newton's method. 
% \end{proposition}
% \begin{proposition}
%     Consider a solution trajectory $\{x,u,\eta,\psi,\lambda,\mu,\gamma\}$ and a set of high-order strategies $\{\pi_t^i\}_{t=0,i=1}^{T,N}$. The associated Quasi policy and high-order policy satisfy
%     \begin{equation}
%         \begin{aligned}
%             a
%         \end{aligned}
%     \end{equation}
% \end{proposition}



% \begin{remark}
%     To bound $\|u_t - u_t^*\|$, we first need to bound $\|(\nabla K)^{-1} - (\nabla K^*)^{-1} \|$. Furthermore, we need to bound $\|\nabla K - \nabla K^*\|$. 
% \end{remark}

% \begin{equation}
%     \begin{aligned}
%         \nabla K(\nabla \pi, u) = 0
%     \end{aligned}
% \end{equation}

% \begin{equation}
%     \begin{aligned}
%         \nabla K(\nabla \pi^*, u^*) = 0
%     \end{aligned}
% \end{equation}
% Suppose that $\|\nabla \pi - \nabla \pi^*\|\le \epsilon$, then 

% Observe that $\pi_t^i = (\nabla K_t^i)^{-1}$, and $\nabla \pi_t^i = $



==> siam_tex/must_read.tex <==
1. (3.5) - (3.12) define global policies?
2. % L_t^i definition, \psi_t^i and \eta_t^i coincide!
3. Add Haimin's reference




1. check new notation consistency
2. change all \pi to \pi^*?





